Mapping NP-Hard Problems to Restricted Adiabatic Quantum Architectures

We introduce a framework for mapping NP-Hard problems to adiabatic quantum computing (AQC) architectures that are heavily restricted in both connectivity and dynamic range of couplings, for which minor-embedding -- the standard problem mapping method -- cannot be directly applied. Separating the mapping into two distinct stages, we introduce problem-specific reductions for both quadratic unconstrained binary optimisation (QUBO) and satisfiability (SAT) and develop the subdivision-embedding method that is suitable for directly embedding onto these heavily restricted architectures. The theory underpinning this framework provides tools to aid in the manipulation of Ising Hamiltonians for the purposes of Ising energy minimisation, and could be used to assist in developing and optimising further problem mapping techniques. For each of the problem mapping methods presented, we examine how the physical qubit count scales with problem size on architectures of varying connectivity.

==> ClauseGadget.tex <==
\begin{tikzpicture}
\node[draw, circle] (a) at (0,0) {} ;
\node[draw, circle] (b) at (1cm,0) {};
\node[draw, circle] (c) at ( 0.5cm,.8cm) {};
\draw[line width=1.2] (a) -- (b);
\draw[line width=1.2] (b) -- (c);
\draw[line width=1.2] (c) -- (a);

\draw[line width=1.2, dashed] (a) -- (-0.2cm, 1.3cm);
\draw[line width=1.2, dashed] (b) -- (1.2cm, 1.3cm);
\draw[line width=1.2, dashed] (c) -- (0.5cm, 1.3cm);

\node[draw, circle] (2a) at (2cm,0) {};
\node[draw, circle] (2b) at (3cm,0) {};
\node[draw, circle] (2c) at (2.5cm, .8cm) {};
\draw[line width = 1.2] (2a) -- (2b);
\draw[line width = 1.2] (2b) -- (2c);
\draw[line width = 1.2] (2c) -- (2a);
\draw[line width = 1.2] (b) -- (2a);

\node[draw, circle] (3a) at (4cm,0) {};
\node[draw, circle] (3b) at (5cm,0) {};
\node[draw, circle] (3c) at (4.5cm, .8cm) {};
\draw[line width = 1.2] (3a) -- (3b);
\draw[line width = 1.2] (3b) -- (3c);
\draw[line width = 1.2] (3c) -- (3a);
\draw[line width = 1.2] (2b) -- (3a);


\end{tikzpicture}

==> HamiltonianGraphCorrespondence.tex <==
\begin{tikzpicture}

  \node at (0,0) {};
  \node at (1,0) {};
  \node at (0,1) {};
  \node at (1,1) {};

  \draw (0,0) -- (1,1);

\end{tikzpicture}

==> LogicalIsing.tex <==
\begin{tikzpicture}

	\tikzstyle{dashdotted}=[dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt]

	\definecolor{var1}{RGB}{102,194,165}
	\definecolor{var2}{RGB}{252,141,98}
	\definecolor{var3}{RGB}{141,160,203}
	\definecolor{var4}{RGB}{231,138,195}

	%CLAUSE GADGETS
	\node[fill=black, draw, circle, scale=0.5] (11) at (-3.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (12) at (-3.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (13) at (-3.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (21) at (-2.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (22) at (-2.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (23) at (-2.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (31) at (-1.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (32) at (-1.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (33) at (-1.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (41) at (-0.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (42) at (-0.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (43) at (-0.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (51) at (0.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (52) at (0.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (53) at (0.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (61) at (1.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (62) at (1.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (63) at (1.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (71) at (2.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (72) at (2.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (73) at (2.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (81) at (3.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (82) at (3.5,0.5) {};
	\node [fill=black, draw,circle, scale=0.5] (83) at (3.75,0) {};
	\node[fill=black, draw, circle, scale=0.5] (91) at (4.25,0) {};
	\node[fill=black, draw, circle, scale=0.5] (92) at (4.5,0.5) {};
	\node[fill=black, draw, circle, scale=0.5] (93) at (4.75,0) {};
	\draw[, line width = 1.1] (11) -- (12);
	\draw[, line width = 1.1] (12) -- (13);
	\draw[, line width = 1.1] (11) -- (13);
	\draw[, line width = 1.1] (21) -- (22);
	\draw[, line width = 1.1] (22) -- (23);
	\draw[, line width = 1.1] (23) -- (21);
	\draw[, line width = 1.1] (31) -- (32);
	\draw[, line width = 1.1] (32) -- (33);
	\draw[, line width = 1.1] (33) -- (31);
	\draw[, line width = 1.1] (41) -- (42);
	\draw[, line width = 1.1] (42) -- (43);
	\draw[, line width = 1.1] (43) -- (41);
	\draw[, line width = 1.1] (51) -- (52);
	\draw[, line width = 1.1] (52) -- (53);
	\draw[, line width = 1.1] (53) -- (51);
	\draw[, line width = 1.1] (61) -- (62);
	\draw[, line width = 1.1] (62) -- (63);
	\draw[, line width = 1.1] (63) -- (61);
	\draw[, line width = 1.1] (71) -- (72);
	\draw[, line width = 1.1] (72) -- (73);
	\draw[, line width = 1.1] (73) -- (71);
	\draw[, line width = 1.1] (81) -- (82);
	\draw[, line width = 1.1] (82) -- (83);
	\draw[, line width = 1.1] (83) -- (81);
	\draw[, line width = 1.1] (91) -- (92);
	\draw[, line width = 1.1] (92) -- (93);
	\draw[, line width = 1.1] (93) -- (91);	
	%INTER-TRIANGLE CONNECTION
	\draw[, line width = 1.1] (23) -- (31);
	\draw[, line width = 1.1] (63) -- (71);
	\draw[, line width = 1.1] (83) -- (91);
	
	
	%VARIABLE-GADGETS
	\node[fill = var1, draw, circle, scale=0.5] (x1) at (-2.5,1.25) {};
	\node[fill = var1, draw, circle, scale=0.5] (nx1) at (-1.75,1.25) {};
	\node[fill = var2, draw, circle, scale=0.5] (x2) at (-0.75,1.25) {};
	\node[fill = var2, draw, circle, scale=0.5] (nx2) at (0,1.25) {};
	\node[fill = var3, draw, circle, scale=0.5] (x3) at (1,1.25) {};
	\node[fill = var3, draw, circle, scale=0.5] (nx3) at (1.75,1.25) {};
	\node[fill = var4, draw, circle, scale=0.5] (x4) at (2.75,1.25) {};
	\draw[var1, line width = 1.1] (x1) -- (nx1);
	\draw[var2, line width = 1.1] (x2) -- (nx2);
	\draw[dashed, var3, line width = 1.1] (x3) -- (nx3);
	\draw[var1, line width = 1.1] (x1) -- (12);
	\draw[var1, line width = 1.1] (x1) -- (61);
	\draw[var1, line width = 1.1] (nx1) -- (22);
	\draw[var1, line width = 1.1] (nx1) -- (42);
	\draw[var2, line width = 1.1] (x2) -- (13);
	\draw[var2, line width = 1.1] (x2) -- (51);
	\draw[var2, line width = 1.1] (nx2) -- (32);
	\draw[var2, line width = 1.1] (nx2) -- (81);
	\draw[dashed, var3, line width = 1.1] (x3) to[out=210, in=15] (33);
	\draw[var3, line width = 1.1] (x3) -- (52);
	\draw[var3, line width = 1.1] (nx3) -- (62);
	\draw[dashed, var3, line width = 1.1] (nx3) -- (82);
	\draw[var4, line width = 1.1] (x4) -- (43);
	\draw[var4, line width = 1.1] (x4) -- (72);
	\draw[dashed, var4, line width = 1.1] (x4) -- (92);
	
	\node at (-2.125,1.5) {$x_1$};
	\node at (-0.375,1.5) {$x_2$};
	\node at (1.375,1.5) {$x_3$};
	\node at (2.75,1.5) {$x_4$};
	
	%VARIABLE Z
	\node[fill=gray!70, draw, circle, scale=0.5] (z1) at (-2.75,-0.5) {};
	\node[fill=gray!70, draw, circle, scale=0.5] (z2) at (-0.75,-0.5) {};
	\node[fill=gray!70, draw, circle, scale=0.5] (z3) at (0.75,-0.5) {};
	\node[fill=gray!70, draw, circle, scale=0.5] (z4) at (2.75,-0.5) {};
	\draw[gray!70, dashed, line width = 1.1] (z1) -- (z2);
	\draw[gray!70, dashed, line width = 1.1] (z2) -- (z3);
	\draw[gray!70, dashed, line width = 1.1] (z3) -- (z4);
	\draw[gray!70, line width = 1.1] (z1) to[out=180, in = -60] (11);
	\draw[gray!70, line width = 1.1] (z1) -- (21);
	\draw[gray!70, line width = 1.1] (z2) -- (41);
	\draw[gray!70, line width = 1.1] (z3) -- (53);
	\draw[gray!70, line width = 1.1] (z4) -- (73);
	\draw[gray!70, line width = 1.1] (z4) to[out=0, in=-140] (93);
	
	\node at (0, -.8) {$z$};



\end{tikzpicture}

==> MaxCut.tex <==
\begin{tikzpicture}

	\definecolor{var1}{RGB}{102,194,165}
	\definecolor{var2}{RGB}{252,141,98}
	\definecolor{var3}{RGB}{141,160,203}
	\definecolor{var4}{RGB}{231,138,195}

	\node[scale = 0.5, draw, circle, fill=var1, label = {[shift={(0,-0.05)}]$x_1$}] (x1) at (-4.25,1.5) {};
	\node[scale = 0.5, draw, circle, label= {[shift={(0,-0.05)}]$\overline{x}_1$}] (nx1) at (-3.75,1.5) {};
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(0,-0.05)}]$a_1$}] (a1) at (-3.25,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$\overline{a}_1$}] (na1) at (-2.75,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$x_2$}] (x2) at (-2.25,1.5) {};
	\node[scale = 0.5, draw, circle, fill=var2, label = {[shift={(0,-0.05)}]$\overline{x}_2$}] (nx2) at (-1.75,1.5) {};
	\node[scale = 0.5, draw, circle, fill=black, label= {[shift={(0,-0.05)}]$a_2$}] (a2) at (-1.25,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$\overline{a}_2$}] (na2) at (-0.75,1.5) {};
	\node[scale = 0.5, draw, circle, fill=var3, label = {[shift={(0,-0.05)}]$x_2$}] (x3) at (-.25,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$\overline{x}_3$}] (nx3) at (.25,1.5) {};
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(0,-0.05)}]$a_3$}] (a3) at (0.75,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$\overline{a}_3$}] (na3) at (1.25,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$x_4$}] (x4) at (1.75,1.5) {};
	\node[scale = 0.5, draw, circle, fill=var4, label = {[shift={(0,-0.05)}]$\overline{x}_4$}] (nx4) at (2.25,1.5) {};
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(0,-0.05)}]$a_4$}] (a4) at (2.75,1.5) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(0,-0.05)}]$\overline{a}_4$}] (na4) at (3.25,1.5) {};
	
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(0,-0.05)}]$\overline{z}_1$}] (nz1) at (-3,-0.6) {};
	\node[scale = 0.5, draw, circle, label ={[shift={(0.2,-0.05)}]$z_1$}] (z1) at (-2.25,-0.6) {};
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(0,-0.05)}]$\overline{z}_2$}] (nz2) at (-1.5,-0.6) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(-0.1,-0.05)}]$z_2$}] (z2) at (-0.75,-0.6) {};
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(-0.1,-0.05)}]$\overline{z}_3$}] (nz3) at (0.75,-0.6) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(-0.15,-0.05)}]$z_3$}] (z3) at (1.5,-0.6) {};
	\node[scale = 0.5, draw, circle, fill=black, label = {[shift={(-0.1,-0.05)}]$\overline{z}_4$}] (nz4) at (2.25,-0.6) {};
	\node[scale = 0.5, draw, circle, label = {[shift={(-0.1,-0.05)}]$z_4$}] (z4) at (3,-0.6) {};
	
	\node[scale = 0.5, draw, circle, fill=black] (zz1)  at (-2.25,-1) {};
	\node[scale = 0.5, draw, circle] (zz2) at (-1.5,-1) {};
	\node[scale = 0.5, draw, circle, fill=black] (zz3) at (-0.25,-1) {};
	\node[scale = 0.5, draw, circle] (zz4) at (0.25,-1) {};
	\node[scale = 0.5, draw, circle, fill=black] (zz5) at (1.5,-1) {};
	\node[scale = 0.5, draw, circle] (zz6) at (2.25,-1) {};

	
	\node[scale = 0.5, draw, circle] (11) at (-3.75,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (12) at (-3.5,0.5) {};
	\node [scale = 0.5, draw,circle] (13) at (-3.25,0) {};
	\node[scale = 0.5, draw, circle] (21) at (-2.75,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (22) at (-2.5,0.5) {};
	\node [scale = 0.5, draw,circle] (23) at (-2.25,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (31) at (-1.75,0) {};
	\node[scale = 0.5, draw, circle] (32) at (-1.5,0.5) {};
	\node [scale = 0.5, draw,circle] (33) at (-1.25,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (41) at (-0.75,0) {};
	\node[scale = 0.5, draw, circle] (42) at (-0.5,0.5) {};
	\node [scale = 0.5, draw,circle] (43) at (-0.25,0) {};
	
	\node[scale = 0.5, draw, circle] (51) at (0.25,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (52) at (0.5,0.5) {};
	\node [scale = 0.5, draw,circle] (53) at (0.75,0) {};
	\node[scale = 0.5, draw, circle] (61) at (1.25,0) {};
	\node[scale = 0.5, draw, circle] (62) at (1.5,0.5) {};
	\node [scale = 0.5, draw,circle, fill=black] (63) at (1.75,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (71) at (2.25,0) {};
	\node[scale = 0.5, draw, circle] (72) at (2.5,0.5) {};
	\node [scale = 0.5, draw,circle] (73) at (2.75,0) {};
	\node[scale = 0.5, draw, circle, fill=black] (81) at (3.25,0) {};
	\node[scale = 0.5, draw, circle] (82) at (3.5,0.5) {};
	\node [scale = 0.5, draw,circle] (83) at (3.75,0) {};
	
	\draw (11) -- (12);
	\draw (12) -- (13);
	\draw (11) -- (13);
	\draw (21) -- (22);
	\draw (22) -- (23);
	\draw (23) -- (21);
	\draw (31) -- (32);
	\draw (32) -- (33);
	\draw (33) -- (31);
	\draw (41) -- (42);
	\draw (42) -- (43);
	\draw (43) -- (41);
	\draw (51) -- (52);
	\draw (52) -- (53);
	\draw (53) -- (51);
	\draw (61) -- (62);
	\draw (62) -- (63);
	\draw (63) -- (61);
	\draw (71) -- (72);
	\draw (72) -- (73);
	\draw (73) -- (71);
	\draw (81) -- (82);
	\draw (82) -- (83);
	\draw (83) -- (81);
	
	\draw[var1, line width=1.1] (x1) -- (nx1);
	\draw[var2, line width=1.1] (x2) -- (nx2);
	\draw[var3, line width=1.1] (x3) -- (nx3);
	\draw[var4, line width=1.1] (x4) -- (nx4);
	\draw (a1) -- (na1);
	\draw (a2) -- (na2);
	\draw (a3) -- (na3);
	\draw (a4) -- (na4);
	
	\draw[var1, line width=1.1] (x1) -- (11);
	\draw[var1, line width=1.1] (x1) -- (51);
	\draw (a1) -- (13);
	\draw (na1) -- (21);
	\draw[var2, line width=1.1] (x2) -- (12);
	\draw[var3, line width=1.1] (nx3) -- (22);
	\draw[var2, line width=1.1] (nx2) -- (42);
	\draw[var2, line width=1.1] (nx2) -- (82);
	\draw (a2) -- (33);
	\draw (na2) -- (41);
	\draw (a3) -- (53);
	\draw (na3) -- (61);
	\draw (a4) -- (73);
	\draw (na4) -- (81);
	\draw[var1, line width=1.1] (nx1) -- (31);
	\draw[var1, line width=1.1] (nx1) -- (71);
	\draw[var3, line width=1.1] (x3) -- (32);
	\draw[var3, line width=1.1] (x3) -- (62);
	\draw[var4, line width=1.1] (x4) -- (52);
	\draw[var4, line width=1.1] (nx4) -- (72);
	
	\draw (z1) -- (nz1);
	\draw (z2) -- (nz2);
	\draw (z3) -- (nz3);
	\draw (z4) -- (nz4);
	
	\draw (z1) -- (zz1);
	\draw (zz1) -- (zz2);
	\draw (zz2) -- (nz2);
	
	\draw (z2) -- (zz3);
	\draw (zz3) -- (zz4);
	\draw (zz4) -- (nz3);
	
	\draw (z3) -- (zz5);
	\draw (zz5) -- (zz6);
	\draw (zz6) -- (nz4);
	
	\draw (z1) -- (23);
	\draw (z2) -- (43);
	\draw (z3) -- (63);
	\draw (z4) -- (83);


\end{tikzpicture}

==> TikzFigures/2ClauseGadget.tex <==
\begin{tikzpicture}
	\node[draw, circle] (a) at (0,0) {} ;
	\node[draw, circle] (b) at (1cm,0) {};
	\draw[line width=1.2] (a) -- (b);
	
	\draw[black!30, line width=1.2] (a) -- (-0.2cm, .8cm);
	\draw[black!30, line width=1.2] (b) -- (1.2cm, .8cm);
\end{tikzpicture}

==> TikzFigures/VariableGadget.tex <==
\begin{tikzpicture}
	\node[draw, circle] (a) at (0,0) {} ;
	\node[draw, circle] (b) at (1cm,0) {};
	\node[above=0.5mm of a] {$x$};
	\node[above=0.5mm of b] {$\overline{x}$};
	\draw[line width = 1.2] (a) -- (b);
\end{tikzpicture}
